Collaborative Prediction: Tractable Information Aggregation via Agreement

We give efficient "collaboration protocols" through which two parties, who observe different features about the same instances, can interact to arrive at predictions that are more accurate than either could have obtained on their own. The parties only need to iteratively share and update their own label predictions-without either party ever having to share the actual features that they observe. Our protocols are efficient reductions to the problem of learning on each party's feature space alone, and so can be used even in settings in which each party's feature space is illegible to the other-which arises in models of human/AI interaction and in multi-modal learning. The communication requirements of our protocols are independent of the dimensionality of the data. In an online adversarial setting we show how to give regret bounds on the predictions that the parties arrive at with respect to a class of benchmark policies defined on the joint feature space of the two parties, despite the fact that neither party has access to this joint feature space. We also give simpler algorithms for the same task in the batch setting in which we assume that there is a fixed but unknown data distribution. We generalize our protocols to a decision theoretic setting with high dimensional outcome spaces, where parties communicate only "best response actions." Our theorems give a computationally and statistically tractable generalization of past work on information aggregation amongst Bayesians who share a common and correct prior, as part of a literature studying "agreement" in the style of Aumann's agreement theorem. Our results require no knowledge of (or even the existence of) a prior distribution and are computationally efficient. Nevertheless we show how to lift our theorems back to this classical Bayesian setting, and in doing so, give new information aggregation theorems for Bayesian agreement.

==> linear-scratch.tex <==
\section{Linear Functions Satisfy the Weak Learning Condition (Scratch)}
Suppose $\cX_A = \{x \in \mathbb{R}^n : ||x|| \leq 1\}, \cX_B = \{x \in \mathbb{R}^m : ||x|| \leq 1 \sg{2?}\}, \cX = \{x \in \mathbb{R}^{n+m} : ||x|| \leq 1\}$, and $\cY = [0,1]$. For $x \in \cX$ we can write $x = (x_A, x_B)$ for $x_A \in \cX_A$ and $x_B \in \cX_B$. 
Define:
$$\cH_J = \{h(x) = \langle \theta, x \rangle : \theta \in \mathbb{R}^{n+m}, ||\theta|| \leq 1\}$$
$$\cH_A(C) = \{h(x) = \langle \theta, x_a \rangle + c : \theta \in \mathbb{R}^{n}, ||\theta|| \leq C, |c| \leq 1\}$$
$$\cH_B(C) = \{h(x) = \langle \theta, x_b \rangle + c : \theta \in \mathbb{R}^{b}, ||\theta|| \leq C, |c| \leq 1\}$$

$\cH_J$ is defined to be the set of all unit-norm \emph{linear} functions over the join feature space $\cX$ whereas the function classes $\cH_A(C)$ and $\cH_B(C)$ are defined to be $C$-norm \emph{affine} functions which allow for a constant offset $c$, but this is for convenience only --- if we fix a constant coordinate in $\cX_a$ and $\cX_b$, then $\cH_J$ can also represent affine functions. 

\begin{theorem}
    Fix any joint distribution $\cD$ over $\cX \times \cY$. Let $\mu = \E[Y]$ be the label mean over $\cD$. Suppose the best function in $\cH_J$ improves in mean squared error over the best constant prediction by a margin of $\gamma$:
    $$\argmin_{h \in \cH_J}\E[(h(x)-y)^2] \leq \E[(\mu-y)^2] - \gamma$$
    Then for $C = \frac{4}{\gamma}$, there is a function in either $\cH_A(C)$ or $\cH_B(C)$ that improves over the best constant predictor by a margin of $\frac{\gamma^4}{256}$. Either:
    $$\argmin_{h \in \cH_A(C)}\E[(h(x_A)-y)^2] \leq \E[(\mu-y)^2] - \frac{\gamma^4}{256}$$
    or:
        $$\argmin_{h \in \cH_B(C)}\E[(h(x_B)-y)^2] \leq \E[(\mu-y)^2] - \frac{\gamma^4}{256}$$
\end{theorem}
\begin{proof}
 Let $h^*\in \cH_J$ be a model satisfying
 $$\E[(h(x)-y)^2] \leq \E[(\mu-y)^2] - \gamma$$
 We know such a model exists from the hypothesis of the theorem. We can write:
 \begin{eqnarray*}
     \E[(\mu-y)^2] - \E[(h(x)-y)^2] &=& \mu^2 - 2\mu\E[y] + \E[y^2] - \E[h(x)^2] + 2\E[h(x)y] - \E[y^2] \\
     &=& \E[y^2] - \mu^2 - \E[h(x)^2] + 2\E[h(x)y] - \E[y^2] \\
     &=&  2\E[h(x)y] - \mu^2 - \E[h(x)^2] \\
     &\geq& \gamma
 \end{eqnarray*}
 Since $\mu^2$ and $\E[h(x)^2]$ are both non-negative, we can conclude that: 
 $$\E[h(x)y] \geq \frac{\gamma}{2}$$
 Observe that we can write $h(x) = h_A(x_A) + h_B(x_A)$ for some linear functions $h_A \in \cH_A(1)$ and $h_B \in \cH_B(1)$ and so we know that for these functions 
  $$\E[h(x)y] = \E[h_A(x_A)y] + \E[h_B(x_B)y]  \geq \frac{\gamma}{2}$$
  We must therefore have that at least one of the two terms above exceeds $\gamma/4$. Without loss of generality (up to relabeling) let us assume that it is the first term:
  $$\E[h_A(x_A)y] \geq \frac{\gamma}{4}$$
  Now define the function $h'(x) = C h_A(x_A) + \mu$ for $C = \frac{\gamma}{4 \E[(h_A(x_A))^2]}$. Observe that $h'(x) \in \cH_A(C)$.
  We examine the squared error of $h'(x)$. Without loss of generality we can shift both our predictions and the labels so that $\mu = 0$ (this does not affect the squared error). Under this shift we can compute:
 \begin{eqnarray*}
  E[(\mu-y)^2] - \E[(h'(x)-y)^2] &=&2\E[h'(x)y] - \E[h'(x)^2] \\
  &=& 2C\E[h_A(x_A)y]  - C^2\E[(h_A(x_A))^2] \\
  &\geq& \frac{C\gamma}{2} -  C^2\E[(h_A(x_A))^2] \\
  &=& \frac{\gamma^2}{16 \E[(h_A(x_A))^2]}
  \end{eqnarray*}
  where the last inequality follows from the definition of $C$. It remains to upper and lower bound  $\E[(h_A(x_A))^2]$. 
  
  
  First a lower bound. We know:
  \begin{eqnarray*}
      \frac{\gamma}{4} &\leq& \E[h_A(x_A)y] \\
      &\leq& \sqrt{\E[h_a(x_a)^2]\E[y^2]} \\
      &\leq& \sqrt{\E[h_a(x_a)^2]}
  \end{eqnarray*}
  where the second inequality is Cauchy-Schwarz and the third follows from $|y| \leq 1$. 
  Hence we know that 
  $$\E[h_a(x_a)^2] \geq \frac{\gamma^2}{16}$$
  and as a result, $C \leq 4/\gamma$. 
  
  Next an upper bound. Since we know that $||x|| \leq 1$ and $h_A \in \cH_A(C)$, we know that pointwise $h_A(x_A) \leq C$ and hence 
  $$\E[(h_A(x_A))^2] \leq C^2 \leq \frac{16}{\gamma^2}$$
  Therefore we have:
  $$ E[(\mu-y)^2] - \E[(h'(x)-y)^2] \geq \frac{\gamma^4}{256}$$
  which completes the proof.
\end{proof}

\subsection{Alternate proof: Surbhi}
Suppose $\cY = [0,1]$. Let $\cX_1 = \{x_1 \in \mathbb{R}^{d_1}: \|x_1\| \leq 1\}$ and $\cX_2 = \{x_2 \in \mathbb{R}^{d_2}: \|x_2\| \leq 1\}$. Define:
$$\cH_1 = \{w_1^\top x_1 + b_1 : \|w_1\| \leq 1, |b_1| \leq 1\}$$
$$\cH_2 = \{w_2^\top x_2 + b_2 : \|w_2\| \leq 1, |b_2| \leq 1\}$$
$$\cH_J = \{w_1^\top x_1 + w_2^\top x_2 + b : \|w_1\| \leq 1, \|w_2\| \leq 1, |b| \leq 1\}$$.

\begin{theorem}
    Fix any joint distribution $\cD$ over $\cX_1 \times \cX_2 \times \cY$. Suppose the best function in $\cH_J$ improves in mean squared error over the best constant prediction by a margin of $0 \le \gamma \le 1$:
    $$\min_{h \in \cH_J}\E[(h(x)-y)^2] \leq \E[(\mu-y)^2] - \gamma$$
    where $\mu = \E[y]$. Then at least one of the feature sets can produce a weak learner. Specifically, there exists either $h_1 \in \cH_1$ or $h_2 \in \cH_2$ such that:
    $$\E[(h_1(x_1)-y)^2] \leq \E[(\mu-y)^2] - \frac{\gamma^2}{16}$$
    or:
    $$\E[(h_2(x_2)-y)^2] \leq \E[(\mu-y)^2] - \frac{\gamma^2}{16}$$
\end{theorem}

\begin{proof}
We first apply a centering transformation to reduce the problem to the zero-mean case. Define $\bar{y} = y - \mu$ so that $\E[\bar{y}] = 0$, and for any predictor $h(x)$, define $\bar{h}(x) = h(x) - \mu$. The best constant predictor for $\bar{y}$ is 0 with error $\E[(\bar{y})^2] = \text{Var}(y)$, and for any predictor, $\E[(h(x)-y)^2] = \E[(\bar{h}(x)-\bar{y})^2]$.

Let $h_J(x) = w_1^\top x_1 + w_2^\top x_2 + b$ be the optimal predictor in $\cH_J$, and $\bar{h}_J(x) = w_1^\top x_1 + w_2^\top x_2 + (b-\mu)$ its centered version. 

By assumption:
\begin{align*}
\E[(\bar{h}_J(x)-\bar{y})^2] &\leq \E[\bar{y}^2] - \gamma
\end{align*}

Since $\E[\bar{y}] = 0$, we can expand:
\begin{align*}
\E[\bar{y}^2] - \E[(\bar{h}_J(x)-\bar{y})^2] &= -\E[(\bar{h}_J(x))^2] + 2\E[\bar{h}_J(x)\bar{y}] \geq \gamma
\end{align*}

Given that $\E[(\bar{h}_J(x))^2] \geq 0$, we have:
\begin{align*}
\E[\bar{h}_J(x)\bar{y}] &\geq \frac{\gamma}{2}\\
\E[(w_1^\top x_1 + w_2^\top x_2 + (b-\mu))\bar{y}] &\geq \frac{\gamma}{2}\\
\E[w_1^\top x_1 \cdot y] + \E[w_2^\top x_2 \cdot y] &\geq \frac{\gamma}{2}
\end{align*}
The last inequality follows from the fact that $\E[\bar{y}] = 0$, so $\E[(b-\mu)\bar{y}] = (b-\mu)\E[\bar{y}] = 0$. 

For this inequality to hold, at least one term must contribute significantly:
\begin{align*}
\E[w_1^\top x_1 \cdot \bar{y}] \geq \frac{\gamma}{4} \quad \text{or} \quad \E[w_2^\top x_2 \cdot \bar{y}] \geq \frac{\gamma}{4}
\end{align*}

Without loss of generality, assume $\E[w_1^\top x_1 \cdot \bar{y}] \geq \frac{\gamma}{4}$. We construct $h_1(x_1) = \alpha w_1^\top x_1 + \mu$ and corresponding centered predictor $\bar{h}_1(x_1) = \alpha w_1^\top x_1$ for $\alpha = \frac{\gamma}{4}$. Note that $h_1, \bar{h}_1 \in \cH_1$ since $\alpha \|w_1\| \le 1$ since $\alpha \le 1$ and $|\mu| \le 1$ since $\cY = [0,1]$.

We calculate the improvement in error:
\begin{align*}
\E[\bar{y}^2] - \E[(\bar{h}_1(x_1)-\bar{y})^2] &= -\E[(\bar{h}_1(x_1))^2] + 2\E[\bar{h}_1(x_1)\bar{y}] \\
&= -\E[(\alpha w_1^\top x_1)^2] + 2\E[\alpha w_1^\top x_1 \cdot \bar{y}] \\
&= -\alpha^2\E[(w_1^\top x_1)^2] + 2\alpha\E[w_1^\top x_1 \cdot \bar{y}]
\end{align*}

Since $\|w_1\| \leq 1$ and $\|x_1\| \leq 1$, by Cauchy-Schwarz, $|w_1^\top x_1| \leq 1$, which means $\E[(w_1^\top x_1)^2] \leq 1$. Therefore:
\begin{align*}
\E[\bar{y}^2] - \E[(\bar{h}_1(x_1)-\bar{y})^2] &\geq -\alpha^2 + 2\alpha \cdot \frac{\gamma}{4} \\
&= -\alpha^2 + \frac{\alpha\gamma}{2}
\end{align*}

For $\alpha = \frac{\gamma}{4}$:
\begin{align*}
\E[\bar{y}^2] - \E[(\bar{h}_1(x_1)-\bar{y})^2] &\geq -\left(\frac{\gamma}{4}\right)^2 + \frac{\gamma}{4} \cdot \frac{\gamma}{2} \\
&= -\frac{\gamma^2}{16} + \frac{\gamma^2}{8} \\
&= \frac{\gamma^2}{16}
\end{align*}

Removing the normalization with $h_1(x_1) = \alpha w_1^\top x_1 + \mu$, we get:
\begin{align*}
\E[(\mu-y)^2] - \E[(h_1(x_1)-y)^2] = \E[(\bar{y})^2] - \E[(\bar{h}_1(x_1)-\bar{y})^2] \geq \frac{\gamma^2}{16}.
\end{align*}

This completes the proof.
\end{proof}

\subsection{Linear Models Do Not Satisfy Information Substitutes}
\begin{theorem}
Linear models do not universally satisfy the information substitute condition. There exist a distribution $\cD$ for which the condition is violated.
\end{theorem}

\begin{proof}
Here we will construct a counterexample to the information substitutes condition. Let $(X_1, X_2, Y)$ be random variables with:
\begin{align*}
X_1 & = \frac{1}{2} \xi_1 \quad \text{where } \xi_1 \sim \{-1, +1\} \\
X_2 &= X_1 + \frac{\xi_2}{2\rho} \quad \text{where }  \xi_1 \sim \{-1, +1\} \text{ independent of } X_1 \\
Y &= 2\rho(X_2 - X_1) = \xi_2
\end{align*}

\begin{itemize}
\item \textbf{Constant predictor:} The optimal constant is $c^* = \E[Y] = 0$, giving $\E[Y^2] = \E[\xi_2^2] = 1$.

\item \textbf{Predictor using only $X_1$:} The optimal linear predictor has form $h_1^*(X_1) = w_1 X_1$. Computing:
\begin{align*}
w_1 &= \frac{\E[X_1Y]}{\E[X_1^2]} = \frac{\E[X_1\xi_2]}{\E[X_1^2]} = \frac{0}{1/4} = 0
\end{align*}
So $h_1^*(X_1) = 0$, yielding $\E[(h_1^*(X_1)-Y)^2] = \E[\xi_2^2] = 1$.

\item \textbf{Predictor using only $X_2$:} The optimal linear predictor has form $h_2^*(X_2) = w_2 X_2$. Computing:
\begin{align*}
w_2 &= \frac{\text{Cov}(X_2,Y)}{\text{Var}(X_2)} = \frac{\E[X_2Y] - \E[X_2]\E[Y]}{\text{Var}(X_2)} = \frac{\E[X_2\xi_2]}{\E[X_2^2]}
\end{align*}
Since 
\begin{align*}
\E[X_2\xi_2] &= \E\left[\left(X_1+\frac{\xi_2}{2\rho}\right)\xi_2\right] = \E[X_1\xi_2] + \frac{1}{2\rho}\E[\xi_2^2] = \frac{1}{2\rho} \\
\text{Var}(X_2) &= \text{Var}(X_1) + \text{Var}\left(\frac{\xi_2}{2\rho}\right) = \frac{1}{4} + \frac{1}{4\rho^2} = \frac{\rho^2+1}{4\rho^2}
\end{align*}
we get $w_2 = \frac{\frac{1}{2\rho}}{\frac{\rho^2+1}{4\rho^2}} = \frac{2\rho}{\rho^2+1}$. This gives us $h_2^*(X_2) = \frac{2\rho}{\rho^2+1}X_2$, and
\begin{align*}
\E\left[(h_2^*(X_2) - Y)^2\right] & = \E\left[\left(\frac{2\rho}{\rho^2+1}X_2 - \xi_2\right)^2\right] \\
&= \E\left[\left(\frac{2\rho}{\rho^2+1}X_1 + \frac{\xi_2}{\rho^2+1} - \xi_2\right)^2\right] \\
&= \E\left[\left(\frac{2\rho}{\rho^2+1}X_1 - \frac{\rho^2}{\rho^2+1}\xi_2\right)^2\right] \\
&= \frac{4\rho^2}{(\rho^2+1)^2}\E[X_1^2] + \frac{\rho^4}{(\rho^2+1)^2}\E[\xi_2^2] - \frac{4\rho^3}{(\rho^2+1)^2}\E[X_1\xi_2] \\
&= \frac{\rho^2}{(\rho^2+1)^2} + \frac{\rho^4}{(\rho^2+1)^2} \\
&= \frac{\rho^2}{\rho^2+1}
\end{align*}

\item \textbf{Predictor using both features:} Since $Y = 2\rho(X_2 - X_1)$, the optimal predictor is $h_{12}^*(X_1,X_2) = 2\rho X_2 - 2\rho X_1 = \xi_2$, yielding $\E\left[(h_{12}^*(X_1,X_2) - Y)^2\right] = 0$.
\end{itemize}

Now observe that:
\begin{align*}
\E\left[(h_1^*(X_1) - Y)^2\right] - \E\left[(h_{12}^*(X_1,X_2) - Y)^2\right] &= 1 - 0 = 1 \\
\E\left[(c^* - Y)^2\right] - \E\left[(h_2^*(X_2) - Y)^2\right] &= 1 - \frac{\rho^2}{\rho^2+1} = \frac{1}{\rho^2+1}.
\end{align*}
The information substitute condition requires $\E\left[(h_1^*(X_1) - Y)^2\right] - \E\left[(h_{12}^*(X_1,X_2) - Y)^2\right] \leq \E\left[(c^* - Y)^2\right] - \E\left[(h_2^*(X_2) - Y)^2\right]$. However, $\frac{1}{\rho^2+1} < 1$ for all $\rho > 0$, so the condition is violated.
\end{proof}

\subsection{Quadratic Dependence is Optimal for Weak Learning}
The counterexample above demonstrates that weak learnability can be made to not hold for any $\gamma > 0$ by choosing a large enough $\rho$. Since $\E[(c^* - Y)^2] - \E[(h_{12}^*(X_1,X_2) - Y)^2] = 1 > \gamma$ for all $\gamma < 1$ and $\E[(c^* - Y)^2] - \E[(h_1^*(X_1) - Y)^2] = 0$, for weak learnability to hold, we need $\E[(c^* - Y)^2] - \E[(h_2^*(X_2) - Y)^2] = \frac{1}{\rho^2+1} > f(\gamma)$ for some function $f$. Now, if we take $\rho$ sufficiently large, we can make this quantity be arbitrarily close to $0$ and violate this condition. 

In the above example, if we take $\rho$ to be very large, we also blow up the norm of the optimal predictor $h^*_{12}$. Constraining this allows us to achieve weak learnability. 

\begin{theorem}
    For each $\gamma$, there exists a distribution $\mathcal{D}$ such that
    \[
    \min_{h \in \cH_J}\E[(h(X_1, X_2)-Y)^2] \leq \E[(\mu-Y)^2] - \gamma
    \]
    but both
    \[
    \min_{h \in \cH_J}\E[(h_1(X_1)-y)^2] \leq \E[(\mu-y)^2] - \gamma
    \]
\end{theorem}
If we consider the joint class to have norm bound 1 on each feature then, we get that the optimal bounded predictor is $h_{12}(X_1, X_2) = X_2 - X_1 = \frac{\xi_2}{2\rho}$. This gives us 
\begin{align*}
    \E[(h_{12}(X_1, X_2) - Y)^2] = \E\left[\left(\frac{\xi_2}{2\rho} - \xi_2\right)^2\right] = \frac{(2\rho - 1)^2}{4\rho^2}.
\end{align*} 
This gives us
\begin{align*}
    \E\left[(c^* - Y)^2\right] - \E[(h_{12}(X_1, X_2) - Y)^2] = 1 - \frac{(2\rho - 1)^2}{4\rho^2} = \frac{4\rho - 1}{4 \rho^2}
\end{align*}
Recall that the optimal $h_2^*(X_2) = \frac{2\rho}{\rho^2+1} X_2$ which satisfies the norm constraint since $2 \rho \le \rho^2 + 1$. This gives us,
\begin{align*}
    \E\left[(c^* - Y)^2\right] - \E[(h^*_{2}(X_2) - Y)^2] = \frac{1}{\rho^2 + 1} 
\end{align*}

==> multi-dimensional.tex <==

This naturally extends to the $d$-dimensional setting, in which we measure agreement using the $\ell_\infty$ norm: 

\begin{definition}[Agreement Condition in the $d$-dimensional Setting] \label{def:agree-dimensions}
    The agreement condition in the $d-$dimensional setting is the function $\textsc{Agree-dDim}_{\eps}: \Omega_h \times \cY \times \Omega_m \times \cY \to \{0, 1\}$ defined as:
    \begin{align*}
        \textsc{Agree-dDim}_{\eps}(p, y_h,  q, y_m) =
        \begin{cases}
            1, & \text{ if } \|p - q\|_{\infty} < \eps \\
            0, & \text{ otherwise.}
        \end{cases}
    \end{align*}
\end{definition}

\begin{definition}[$d$-dimensional Full Feedback Setting] \label{def:setting-dimensions}
    The $d$-dimensional full feedback setting refers to Protocol \ref{alg:general-agreement} instantiated with $\Omega_h = \Omega_m = \cY = [0,1]^d$, messages $\pmk{t}{k} = \ymk{t}{k}$ and $\phk{t}{k} = \yhk{t}{k}$, and the agreement condition $\textsc{Agree}_{\eps} = \textsc{Agree-dDim}_{\eps}$ (Definition \ref{def:agree-dimensions}).
\end{definition}


\iffalse
\paragraph{Limited (Directional) Feedback}

In this setting, we consider a human who acts in ways consistent with some internal prediction $\hat y_h^t \in \cY = [0,1]$ but may not be able to precisely enunciate their predictions numerically. Instead they  provide a weaker form of feedback to the model.
After seeing the model's most recent prediction, they respond with a judgment of whether the model's prediction is too low, too high, or approximately equal, compared to their underlying estimate. The human's message space will therefore be $\Omega_h = \{ \textsc{Low}, \textsc{High}, \textsc{Equal} \}$. In an $\epsilon$-agreement protocol, they will respond with $\textsc{High}$ when $\hat y_h^t \leq \hat y^t_m - \epsilon$, will respond with $\textsc{Low}$ when $\hat y_h^t \geq \hat y^t_m + \epsilon$, and will respond with $\textsc{Equal}$ otherwise. 

\begin{definition}[Agreement Condition in the Limited Feedback Setting] \label{def:agree-limited}
    The agreement condition in the limited feedback setting is the function $\textsc{Agree-Limited}_{\eps}: \Omega_h \times \cY \times \Omega_m \times \cY \to \{0, 1\}$ defined as:
     \begin{align*}
        \textsc{Agree-Limited}_{\eps}(p, y_h, q, y_m) =
        \begin{cases}
            1, & \text{ if } p = \textsc{Equal} \\
            0, & \text{ otherwise.}
        \end{cases}
    \end{align*}
\end{definition}

\begin{definition}[Limited Feedback Setting] \label{def:setting-limited}
    The limited feedback setting refers to Protocol \ref{alg:general-agreement} instantiated with $\Omega_m = \cY = \mathbb{R}$, $\Omega_h = \{ \textsc{Low}, \textsc{High}, \textsc{Equal} \}$, messages 
    \begin{align*}
        \phk{t}{k} = 
        \begin{cases}
            \textsc{High}, & \text { if } \yhk{t}{k} \leq \ymk{t}{k} - \eps \\
            \textsc{Low}, & \text{ if } \yhk{t}{k} \geq \ymk{t}{k} + \eps \\
            \textsc{Equal} & \text{ otherwise,}
        \end{cases}
    \end{align*} and the agreement condition $\textsc{Agree}_{\eps} = \textsc{Agree-Limited}_{\eps}$ (Definition \ref{def:agree-limited}).
\end{definition}

The limited feedback setting can naturally be extended to $d$ dimensions in which the human provides feedback for each dimension of the prediction, just as we extend the full feedback setting in this way. We omit this generalization out of pity for the reader.  
\fi

% \begin{algorithm}[ht]
% \begin{algorithmic}
%     \STATE{\bf Input} Human $h$, model $m$
%     \STATE{\bf Parameter} {$\epsilon:$ agreement tolerance}
%     \FOR{$t = 1, \ldots, T$}
%         \STATE Receive $x^t = (x^t_h,x^t_m)$
%         \STATE Model sees $x^t_m$ and human sees $x^t_h$ 
%         \FOR{$i = 1, 2, \ldots$}
%             \STATE Model predicts $p_m^t(i)$ 
%             \IF{ $ |p_m^t(i) - p_h^t(i-1)| \leq \epsilon$} 
%             \STATE Predict $p_m^t(i)$ and break out of loop
%             \ENDIF
%             \STATE Human sees $p_m^t(i)$ and reports $p_h^t(i) \in \{\textsc{Low}, \textsc{Equal}, \textsc{High} \}$
%             \IF{ $ p_h^t(i) = \textsc{Equal} $} 
%             \STATE Predict $p_m^t(i)$ and break out of loop
%             \ENDIF
%         \ENDFOR
%     \ENDFOR
%     \STATE{\bf Output} $ \pi = \{ \left[ (p^1_m(1), p^1_h(1)), \ldots (\pmk{1}{i}, \phk{1}{i}), y^1 \right], \ldots \left[ (\pmk{t}{1}, p^T_h(1)), \ldots, (\pmk{t}{i}, \phk{t}{i}), y^T  \right] \}$
% \end{algorithmic}
% \caption{\textsc{Agree-Lim}(h, m) Iterated agreement protocol for binary prediction with limited human feedback} \label{alg:2}
% \end{algorithm}

